Visual Model Validation via Inline Replication

Data visualizations typically show retrospective views of an existing dataset with little or no focus on repeatability. However, consumers of these tools often use insights gleaned from retrospective visualizations as the basis for decisions about future events. In this way, visualizations often serve as visual predictive models despite the fact that they are typically designed to present historical views of the data. This "visual predictive model" approach, however, can lead to invalid inferences. In this paper, we describe an approach to visual model validation called Inline Replication (IR) which, similar to the cross-validation technique used widely in machine learning, provides a nonparametric and broadly applicable technique for visual model assessment and repeatability. This paper describes the overall IR process and outlines how it can be integrated into both traditional and emerging "big data" visualization pipelines. Examples are provided showing IR integrated within common visualization techniques (such as bar charts and linear regression lines) as well as a more fully-featured visualization system designed for complex exploratory analysis tasks.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = paper.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = vast2015.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

pdf:     clean pdftex 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< paper.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< paper.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) paper.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

